Large Deviations for Hamiltonian Systems on Intermediate Time Scales

We consider a two-dimensional Hamiltonian system perturbed by a small diffusion term, whose coefficient is state-dependent and non-degenerate. As a result, the process consists of the fast motion along the level curves and slow motion across them. On finite time intervals, the large deviation principle applies, while on time scales that are inversely proportional to the size of the perturbation, the averaging principle holds, i.e., the projection of the process onto the Reeb graph converges to a Markov process. In our paper, we consider the intermediate time scales and prove the large deviation principle, with the action functional determined in terms of the averaged process on the graph.

==> references.tex <==
@book{nagy,
AUTHOR = {Riesz, Frigyes and Sz.-Nagy, B\'{e}la},
     TITLE = {Functional analysis},
    SERIES = {Dover Books on Advanced Mathematics},
 PUBLISHER = {Dover Publications, Inc., New York},
      YEAR = {1990}
}
@article{semi,    
    AUTHOR = {Liptser, Robert Sh. and Pukhalskii, Anatolii A.},
     TITLE = {Limit theorems on large deviations for semimartingales},
   JOURNAL = {Stochastics Stochastics Rep.},
  FJOURNAL = {Stochastics and Stochastics Reports},
    VOLUME = {38},
      YEAR = {1992},
    NUMBER = {4},
     PAGES = {201--249},
}
@book{shreve,
      AUTHOR = {Karatzas, Ioannis and Shreve, Steven E.},
     TITLE = {Brownian motion and stochastic calculus},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {113},
   EDITION = {Second},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1991}
}
@book {martingale,
    AUTHOR = {Liptser, R. Sh. and Shiryayev, A. N.},
     TITLE = {Theory of martingales},
    SERIES = {Mathematics and its Applications (Soviet Series)},
    VOLUME = {49},
 PUBLISHER = {Kluwer Academic Publishers Group, Dordrecht},
      YEAR = {1989}
}
@book{fred,
    AUTHOR = {Freidlin, Mark I. and Wentzell, Alexander D.},
     TITLE = {Random perturbations of dynamical systems},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {260},
   EDITION = {Third},
 PUBLISHER = {Springer, Heidelberg},
      YEAR = {2012},

}
@article{Hairer2016AFK,
    AUTHOR = {Hairer, Martin and Iyer, Gautam and Koralov, Leonid and
              Novikov, Alexei and Pajor-Gyulai, Zsolt},
     TITLE = {A fractional kinetic process describing the intermediate time
              behaviour of cellular flows},
   JOURNAL = {Ann. Probab.},
  FJOURNAL = {The Annals of Probability},
    VOLUME = {46},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {897--955}
}
@article{Ventsel__1970,
	year = 1970,
	publisher = {{IOP} Publishing},
	volume = {25},
	number = {1},
	pages = {1--55},
	author = {Freidlin, Mark I. and Wentzell, Alexander D.},
	title = {On small random perturbation of dynamical systems},
	journal = {Russian Mathematical Surveys},
}
@article{Liptser1996LargeDF,
    AUTHOR = {Liptser, Robert},
     TITLE = {Large deviations for two scaled diffusions},
   JOURNAL = {Probab. Theory Related Fields},
  FJOURNAL = {Probability Theory and Related Fields},
    VOLUME = {106},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {71--104}
}
@article {MR1883738,
    AUTHOR = {Freidlin, Mark},
     TITLE = {Reaction-diffusion in incompressible fluid: asymptotic
              problems},
   JOURNAL = {J. Differential Equations},
  FJOURNAL = {Journal of Differential Equations},
    VOLUME = {179},
      YEAR = {2002},
    NUMBER = {1},
     PAGES = {44--96}
}
